AutoMixQ: Self-Adjusting Quantization for High Performance Memory-Efficient Fine-Tuning

Fine-tuning large language models (LLMs) under resource constraints is a significant challenge in deep learning. Low-Rank Adaptation (LoRA), pruning, and quantization are all effective methods for improving resource efficiency. However, combining them directly often results in suboptimal performance, especially with uniform quantization across all model layers. This is due to the complex, uneven interlayer relationships introduced by pruning, necessitating more refined quantization strategies. To address this, we propose AutoMixQ, an end-to-end optimization framework that selects optimal quantization configurations for each LLM layer. AutoMixQ leverages lightweight performance models to guide the selection process, significantly reducing time and computational resources compared to exhaustive search methods. By incorporating Pareto optimality, AutoMixQ balances memory usage and performance, approaching the upper bounds of model capability under strict resource constraints. Our experiments on widely used benchmarks show that AutoMixQ reduces memory consumption while achieving superior performance. For example, at a 30\% pruning rate in LLaMA-7B, AutoMixQ achieved 66.21\% on BoolQ compared to 62.45\% for LoRA and 58.96\% for LoftQ, while reducing memory consumption by 35.5\% compared to LoRA and 27.5\% compared to LoftQ.

==> docs/background_old.tex <==
\section{Background and Motivation}
\subsection{Low-Rank Adaptation (LoRA)}\label{sec-bkg-lora}

In the context of structural pruning for LLMs, LoRA fine-tuning is employed to recover performance with minimal parameter updates. For a pruned LLM consisting of $n$ layers, the weight matrices at each layer, denoted as $W$, undergo updates through an update matrix $\Delta W$. This update matrix is decomposed into the product of two low-rank matrices $A$ and $B$, where $A \in \mathbb{R}^{d \times r}$ and $B \in \mathbb{R}^{r \times d}$, with $r$ being the rank, a hyperparameter fixed across all layers. The effectiveness of fine-tuning is critically influenced by the choice of the rank $r$. In this approach, the original weight matrix $W$ remains frozen, while only $\Delta W$, represented by the product $AB$, is updated.
The forward computation can be expressed as:
\begin{equation}
\small
f(x) = (W + \Delta W)X + b = (WX + b) + (AB)X.
\end{equation}
Given the rank $r$ is typically much smaller than the dimension $d$, the number of parameters is significantly reduced from $d^2$ to $2dr$. This optimization can reduce the trainable parameters during the learning.

\subsection{Structural Pruning Framework}\label{2.1}
The structural pruning framework \cite{ma2023llm} is a task-agnostic method for compressing LLMs through three stages: discovery, estimation, and recovery.

\noindent{\textbf{Discovery Stage.}}
This stage identifies clusters of interconnected structures in the LLM. If neuron $N_i$ points to neuron $N_j$ (i.e., $N_j$ is in $\operatorname{Out}(N_i)$) and $N_j$ has an in-degree of one ($\operatorname{Deg}^-(N_j)=1$), $N_j$ is considered dependent on $N_i$:
\begin{equation}\label{equation2}
    \begin{array}{rl}
         N_j & \in \operatorname{Out}(N_i) \wedge \operatorname{Deg}^-(N_j) = 1 \\
         & \Rightarrow N_j \text{ is dependent on } N_i
    \end{array}
\end{equation}
Pruning $N_j$ necessitates pruning $N_i$ due to this dependency, potentially triggering a cascade of activations that identify neuron clusters for pruning.

\noindent{\textbf{Estimation Stage.}}
Once clusters are identified, their impact on model performance is evaluated. For a dataset $\mathcal{D} = {x_i, y_i}{i=1}^N$, and a group $\mathcal{G} = {W_i}{i=1}^M$, the significance $I_{W_i^k}$ of weights $W_i^k$ is assessed using Taylor expansion:
\begin{equation}\label{equation3}
\small
\begin{aligned}
\left| \frac{\partial \mathcal{L}(\mathcal{D})}{\partial W_i^k} W_i^k - \frac{1}{2} \sum_{j=1}^N \left(\frac{\partial \mathcal{L}(\mathcal{D}_j)}{\partial W_i^k} W_i^k\right)^2 + \mathcal{O}\left(| W_i^k |^3\right) \right|
\end{aligned}
\end{equation}
Groups are ranked by importance and those with lower significance are pruned.

\noindent{\textbf{Recovery Stage.}}
Post-pruning, Low-Rank Adaptation (LoRA) fine-tuning is applied to mitigate performance loss and recover the LLM's original performance.

\subsection{Quantization with LoRA}\label{sec-bkg-loftq}
LoftQ (LoRA-Fine-Tuning-aware Quantization) \cite{li2023loftq} is an advanced quantization framework designed to integrate low-rank adaptation with fine-tuned quantization for large language models. It initializes and quantizes the model weights by solving the following optimization problem:

\begin{equation}
\min_{Q,A,B} \| W - Q - AB^T \|_F,
\end{equation}

where $\| \cdot \|_F$ denotes the Frobenius norm. This process involves alternating between quantization and singular value decomposition (SVD). At each step, it first quantizes the residual:

\begin{equation}
Q_t = q_N(W - A_{t-1} B_{t-1}^T),
\end{equation}

and then performs SVD on the quantization residual $R_t = W - Q_t$:

\begin{equation}
R_t = \sum_{i=1}^{d} \sigma_{t,i} u_{t,i} v_{t,i}^T,
\end{equation}

updating the low-rank matrices by selecting the top $r$ singular values and vectors:

\begin{equation}
A_t = [\sqrt{\sigma_{t,1}} u_{t,1}, \ldots, \sqrt{\sigma_{t,r}} u_{t,r}],
\end{equation}
\begin{equation}
B_t = [\sqrt{\sigma_{t,1}} v_{t,1}, \ldots, \sqrt{\sigma_{t,r}} v_{t,r}].
\end{equation}

By alternating these steps, LoftQ effectively reduces the discrepancies introduced by quantization, providing a more accurate initialization for LoRA fine-tuning. This approach significantly improves performance in downstream tasks, particularly under low-bit quantization scenarios. 

\subsection{A Motivating Example}\label{2.4}

Efficient deployment of large language models (LLMs) on resource-constrained devices requires effective model compression and fine-tuning techniques. Structural pruning reduces model size by removing less important parameters, but it often results in uneven pruning across different layers due to their varying importance \cite{zhang2023adalora}. This uneven pruning results in a complex network structure, and standard fine-tuning methods, which typically apply a uniform approach to all layers, may not be the best choice.

We conduct experiments using llama-7b with a 20\% pruning rate. The fine-tuning configurations are as follows: 1) a uniform 16-bit setting for all layers, 2) a uniform 8-bit quantization for all layers, and 3) a mixed-precision setting where each layer is randomly assigned a quantization bit-width of either 4 or 8 bits. The results show that mixed-precision quantization reduces memory consumption while maintaining good task accuracy (Table \ref{tab:task accuracy}).

\begin{table*}[t]
    \centering
    \resizebox{0.86\textwidth}{!}{\begin{tabular}{@{}llcccccccc@{}}
        \toprule
        Pruning Rate &  & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA & Memory (GB)  \\
        \midrule
        \multirow{3}{*}{Rate = 20\%} 
         & LoRA  & 63.30 & \textbf{76.82} & \textbf{68.68} & \textbf{63.38} & 63.76 & 37.11 & \textbf{40.60} & 26.10 \\
         & LoftQ & \textbf{67.37} & 76.71 &68.08 & 61.48 & 65.03 & 38.05 & 39.40 & 18.90 \\
         & LoftQ* & 66.42 & 76.66 & 67.96 & 60.93 & \textbf{66.16} & \textbf{38.40} & 40.00 & \textbf{16.81}  \\
         \bottomrule
        \end{tabular}}
\caption{Overall performance of seven benchmarks
for the different fine-tuning configurations. LoftQ denotes using uniform 8-bit quantization for all layers, whereas
LoftQ* indicates using mixed-precision quantization.}
\label{tab:task accuracy}
\end{table*}



